On Nearest Neighbors in Non Local Means Denoising

To denoise a reference patch, the Non-Local-Means denoising filter processes a set of neighbor patches. Few Nearest Neighbors (NN) are used to limit the computational burden of the algorithm. Here here we show analytically that the NN approach introduces a bias in the denoised patch, and we propose a different neighbors' collection criterion, named Statistical NN (SNN), to alleviate this issue. Our approach outperforms the traditional one in case of both white and colored noise: fewer SNNs generate images of higher quality, at a lower computational cost.

==> Tables/Avg_05.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
image & Noisy & NN & SNN & PSNR-NN & PSNR-SNN & MSSSIM-NN & MSSSIM-SNN \\
\hline
PSNR & 34.15 & 38.00 & 38.19 & 38.00 & \bf{38.19} & 37.96 & 38.14\\
SSIM & 0.9623 & 0.9837 & 0.9841 & 0.9837 & 0.9841 & 0.9839 & \bf{0.9843}\\
MSSSIM & 0.9795 & 0.9913 & 0.9916 & 0.9913 & 0.9915 & 0.9914 & \bf{0.9917}\\
\hline
\end{tabular}
\caption{Average image quality metrics measured on the testing dataset for ANLM, $\sigma = 5$. In bold, the best metric for each row.}
\label{table:05}
\end{center}
\end{table}


==> Tables/Avg_20.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
image & Noisy & NN & SNN & PSNR-NN & PSNR-SNN & MSSSIM-NN & MSSSIM-SNN \\
\hline
PSNR & 22.11 & 29.15 & 30.79 & 30.13 & \bf{30.85} & 29.91 & 30.42\\
SSIM & 0.6750 & 0.8725 & 0.8985 & 0.8935 & 0.9035 & 0.8958 & \bf{0.9075}\\
 MSSSIM & 0.8191 & 0.9296 & 0.9431 & 0.9409 & 0.9467 & 0.9419 & \bf{0.9488}\\
\hline
\end{tabular}
\caption{Average image quality metrics measured on the testing dataset for ANLM, $\sigma = 20$. In bold, the best metric for each row.}
\label{table:20}
\end{center}
\end{table}


==> Tables/Avg_40.tex <==
\begin{table}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
image & Noisy & NN & SNN & PSNR-NN & PSNR-SNN & MSSSIM-NN & MSSSIM-SNN \\
\hline
PSNR & 16.09 & 25.31 & 27.36 & 25.33 & \bf{27.38} & 25.91 & 27.12\\
SSIM & 0.4155 & 0.7374 & 0.7981 & 0.7369 & 0.7976 & 0.7677 & \bf{0.8065}\\
 MSSSIM & 0.6296 & 0.8488 & 0.8752 & 0.8485 & 0.8749 & 0.8649 & \bf{0.8820}\\
\hline
\end{tabular}
\caption{Average image quality metrics measured on the testing dataset for ANLM, $\sigma = 40$. In bold, the best metric for each row.}
\label{table:40}
\end{center}
\end{table}


==> Tables/Grey_Sigma510.tex <==
\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|l||c|c|c|c|c|}
\hline
& \multicolumn{5}{|c|}{$\sigma = 5$} \\
\hline
 & PSNR & SSIM & MSSSIM & GMSD & FSIM\\
\hline
Noisy & 34.15 & 0.8487 & 0.9775 & 0.0222 & 0.9447\\
\hline
o = 0 & 36.22 & 0.9142 & 0.9866 & 0.0142 & 0.9660\\
\hline
o = 0.1 & 36.34 & 0.9174 & 0.9870 & 0.0141 & 0.9667\\
%o = 0.2 & 36.46 & 0.9206 & 0.9873 & \bf{0.0139} & 0.9674 & 31.51 & 0.7922 & 0.9610 & 0.0398 & 0.9169\\
o = 0.35 & 36.63 & 0.9252 & 0.9878 & \bf{0.0139} & 0.9681\\
%o = 0.5 & 36.79 & 0.9296 & 0.9882 & 0.0140 & \bf{0.9685} & 32.10 & 0.8212 & 0.9649 & 0.0376 & 0.9238\\
o = 0.65 & 36.93 & 0.9334 & 0.9885 & 0.0143 & \bf{0.9683}\\
o = 0.8 & 37.03 & 0.9366 & \bf{0.9886} & 0.0149 & 0.9676\\
o = 0.9 & 37.08 & 0.9381 & \bf{0.9886} & 0.0154 & 0.9666\\
o = 1.0 & \bf{37.09} & \bf{0.9392} & 0.9885 & 0.0161 & 0.9652\\
\hline
\hline
& \multicolumn{5}{|c|}{$\sigma = 10$} \\
\hline
 & PSNR & SSIM & MSSSIM & GMSD & FSIM\\
\hline
Noisy & 28.13 & 0.6267 & 0.9263 & 0.0702 & 0.8497\\
\hline
o = 0 & 31.13 & 0.7735 & 0.9581 & 0.0418 & 0.9114\\
\hline
o = 0.1 & 31.32 & 0.7827 & 0.9596 & 0.0407 & 0.9142\\
%o = 0.2 & 36.46 & 0.9206 & 0.9873 & \bf{0.0139} & 0.9674 & 31.51 & 0.7922 & 0.9610 & 0.0398 & 0.9169\\
o = 0.35 & 31.80 & 0.8067 & 0.9631 & 0.0385 & 0.9207\\
%o = 0.5 & 36.79 & 0.9296 & 0.9882 & 0.0140 & \bf{0.9685} & 32.10 & 0.8212 & 0.9649 & 0.0376 & 0.9238\\
o = 0.65 & 32.37 & 0.8351 & 0.9666 & \bf{0.0372} & 0.9259\\
o = 0.8 & 32.62 & 0.8477 & 0.9678 & 0.0373 & \bf{0.9267}\\
o = 0.9 & 32.75 & 0.8550 & 0.9684 & 0.0378 & 0.9262\\
o = 1.0 & \bf{32.86} & \bf{0.8610} & \bf{0.9687} & 0.0387 & 0.9248\\
\hline
\end{tabular}
\normalsize
\caption{Image quality metrics for denoising the gray-level Kodak dataset, corrupted by zero-mean Gaussian noise, $\sigma~=~\{5,~10\}$, using a bilateral filter and different offsets $o$ for the range weights. The case $o = 0$ corresponds to the traditional bilateral filter.}
\label{tab:bilateral}
\end{center}
\vspace{-1em}
\end{table}

%\begin{table*}
%\begin{center}
%\scriptsize
%\begin{tabular}{|l||c|c|c|c|c||c|c|c|c|c|}
%\hline
%& \multicolumn{5}{|c||}{$\sigma = 5$} & \multicolumn{5}{|c|}{$\sigma = 10$} \\
%\hline
% & PSNR & SSIM & MSSSIM & GMSD & FSIM & PSNR & SSIM & MSSSIM & GMSD & FSIM \\
%\hline
%Noisy & 34.15 & 0.8487 & 0.9775 & 0.0222 & 0.9447 & 28.13 & 0.6267 & 0.9263 & 0.0702 & 0.8497\\
%\hline
%o = 0 & 36.22 & 0.9142 & 0.9866 & 0.0142 & 0.9660 & 31.13 & 0.7735 & 0.9581 & 0.0418 & 0.9114\\
%\hline
%o = 0.1 & 36.34 & 0.9174 & 0.9870 & 0.0141 & 0.9667 & 31.32 & 0.7827 & 0.9596 & 0.0407 & 0.9142\\
%%o = 0.2 & 36.46 & 0.9206 & 0.9873 & \bf{0.0139} & 0.9674 & 31.51 & 0.7922 & 0.9610 & 0.0398 & 0.9169\\
%o = 0.35 & 36.63 & 0.9252 & 0.9878 & \bf{0.0139} & 0.9681 & 31.80 & 0.8067 & 0.9631 & 0.0385 & 0.9207\\
%%o = 0.5 & 36.79 & 0.9296 & 0.9882 & 0.0140 & \bf{0.9685} & 32.10 & 0.8212 & 0.9649 & 0.0376 & 0.9238\\
%o = 0.65 & 36.93 & 0.9334 & 0.9885 & 0.0143 & \bf{0.9683} & 32.37 & 0.8351 & 0.9666 & \bf{0.0372} & 0.9259\\
%o = 0.8 & 37.03 & 0.9366 & \bf{0.9886} & 0.0149 & 0.9676 & 32.62 & 0.8477 & 0.9678 & 0.0373 & \bf{0.9267}\\
%o = 0.9 & 37.08 & 0.9381 & \bf{0.9886} & 0.0154 & 0.9666 & 32.75 & 0.8550 & 0.9684 & 0.0378 & 0.9262\\
%o = 1.0 & \bf{37.09} & \bf{0.9392} & 0.9885 & 0.0161 & 0.9652 & \bf{32.86} & \bf{0.8610} & \bf{0.9687} & 0.0387 & 0.9248\\
%\hline
%\end{tabular}
%\normalsize
%\vspace{-0.8em}
%\caption{Image quality metrics for denoising the gray-level Kodak dataset, corrupted by zero-mean Gaussian noise, $\sigma~=~\{5,~10\}$, using a bilateral filter and different offsets $o$ for the range weights.}
%\label{tab:bilateral}
%\end{center}
%\end{table*}


==> Tables/NLM_sigma05.tex <==
\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 & PSNR & SSIM & MSSSIM & GMSD & FSIM & FSIM$_C$ \\
\hline
noisy & 34.15 & .9625 & .9797 & .0211 & .9937 & .9931\\
\hline
NLM$^{361}_{0.0}$ & 38.34 & .9851 & .9921 & .0130 & .9941 & .9939\\
NLM$^{16}_{0.0}$ & 38.08 & .9847 & .9919 & .\bf{0113} & \bf{.9949} & \bf{0.9947}\\
\hline
NLM$^{16}_{0.1}$ & 38.08 & .9847 & .9919 & \bf{.0113} & \bf{.9949} & \bf{0.9947}\\
NLM$^{16}_{0.2}$ & 38.08 & .9847 & .9919 & \bf{.0113} & \bf{.9949} & \bf{0.9947}\\
NLM$^{16}_{0.35}$ & 38.08 & .9847 & .9919 & \bf{.0113} & \bf{.9949} & \bf{0.9947}\\
NLM$^{16}_{0.5}$ & 38.09 & .9848 & .9919 & \bf{.0113} & \bf{.9949} & \bf{0.9947}\\
NLM$^{16}_{0.65}$ & 38.14 & .9850 & .9920 & \bf{.0113} & \bf{.9949} & \bf{0.9947}\\
NLM$^{16}_{0.8}$ & 38.23 & \bf{.9854} & .9922 & .0115 & .9948 & .9946\\
NLM$^{16}_{0.9}$ & 38.28 & \bf{.9854} & \bf{.9923} & .0118 & .9946 & .9945\\
NLM$^{16}_{1.0}$ & \bf{38.29} & .9852 & .9921 & .0124 & .9944 & .9942\\
\hline
\end{tabular}
\normalsize
\caption{Average image quality index for Gaussian noise, $\sigma=5$.}
\label{table:NLM_sigma05}
\end{center}
\end{table}


==> Tables/NLM_sigma10.tex <==
\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 & PSNR & SSIM & MSSSIM & GMSD & FSIM & FSIM$_C$ \\
\hline
noisy & 28.1292 & 0.8744 & 0.9332 & 0.0667 & 0.9763 & 0.9743\\
\hline
NLM$^{361}_{0.0}$ & 34.8354 & 0.9634 & 0.9804 & 0.0338 & 0.9814 & 0.9811\\
NLM$^{16}_{0.0}$ & 33.9589 & 0.9580 & 0.9773 & 0.0269 & \bf{0.9861} & 0.9856\\
\hline
NLM$^{16}_{0.1}$ & 33.9589 & 0.9580 & 0.9773 & 0.0269 & \bf{0.9861} & 0.9856\\
NLM$^{16}_{0.2}$ & 33.9589 & 0.9580 & 0.9773 & 0.0269 & \bf{0.9861} & 0.9856\\
NLM$^{16}_{0.35}$ & 33.9590 & 0.9580 & 0.9773 & 0.0269 & \bf{0.9861} & 0.9856\\
NLM$^{16}_{0.5}$ & 33.9893 & 0.9584 & 0.9775 & 0.0268 & \bf{0.9861} & \bf{0.9857}\\
NLM$^{16}_{0.65}$ & 34.1906 & 0.9610 & 0.9789 & \bf{0.0266} & \bf{0.9861} & \bf{0.9857}\\
NLM$^{16}_{0.8}$ & 34.5072 & 0.9639 & 0.9805 & 0.0274 & 0.9856 & 0.9852\\
NLM$^{16}_{0.9}$ & 34.6635 & \bf{0.9645} & \bf{0.9809} & 0.0291 & 0.9845 & 0.9841\\
NLM$^{16}_{1.0}$ & \bf{34.7128} & 0.9635 & 0.9803 & 0.0319 & 0.9828 & 0.9824\\
\hline
\end{tabular}
\normalsize
\caption{Average image quality index for Gaussian noise, $\sigma=10$.}
\label{table:NLM_sigma10}
\end{center}
\end{table}


==> Tables/NLM_sigma20.tex <==
\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 & PSNR & SSIM & MSSSIM & GMSD & FSIM & FSIM$_C$ \\
\hline
noisy & 22.1108 & 0.6810 & 0.8236 & 0.1549 & 0.9250 & 0.9174\\
\hline
NLM$^{361}_{0.0}$ & \bf{31.1844} & 0.9109 & 0.9505 & 0.0749 & 0.9475 & 0.9468\\
NLM$^{16}_{0.0}$ & 29.2126 & 0.8802 & 0.9343 & 0.0607 & 0.9646 & 0.9633\\
\hline
NLM$^{16}_{0.1}$ & 29.2126 & 0.8802 & 0.9343 & 0.0607 & 0.9646 & 0.9633\\
NLM$^{16}_{0.2}$ & 29.2126 & 0.8802 & 0.9343 & 0.0607 & 0.9646 & 0.9633\\
NLM$^{16}_{0.35}$ & 29.2130 & 0.8802 & 0.9343 & 0.0607 & 0.9646 & 0.9633\\
NLM$^{16}_{0.5}$ & 29.2888 & 0.8826 & 0.9356 & 0.0600 & 0.9648 & 0.9635\\
NLM$^{16}_{0.65}$ & 29.7477 & 0.8948 & 0.9420 & \bf{0.0572} & \bf{0.9653} & \bf{0.9641}\\
NLM$^{16}_{0.8}$ & 30.4531 & 0.9086 & 0.9493 & 0.0583 & 0.9631 & 0.9621\\
NLM$^{16}_{0.9}$ & 30.8088 & \bf{0.9119} & \bf{0.9511} & 0.0635 & 0.9585 & 0.9576\\
NLM$^{16}_{1.0}$ & 30.9263 & 0.9084 & 0.9490 & 0.0719 & 0.9510 & 0.9503\\
\hline
\end{tabular}
\normalsize
\caption{Average image quality index for Gaussian noise, $\sigma=20$.}
\label{table:NLM_sigma20}
\end{center}
\end{table}


==> Tables/NLM_sigma30.tex <==
\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 & PSNR & SSIM & MSSSIM & GMSD & FSIM & FSIM$_C$ \\
\hline
noisy & 18.5914 & 0.5331 & 0.7243 & 0.2138 & 0.8687 & 0.8536\\
\hline
NLM$^{900}_{0.0}$ & \bf{29.1081} & 0.8631 & 0.9197 & 0.1071 & 0.9154 & 0.9144\\
NLM$^{16}_{0.0}$ & 27.3964 & 0.8273 & 0.9035 & 0.0827 & 0.9438 & 0.9419\\
\hline
NLM$^{16}_{0.1}$ & 27.3964 & 0.8273 & 0.9035 & 0.0827 & 0.9438 & 0.9419\\
NLM$^{16}_{0.2}$ & 27.3964 & 0.8273 & 0.9035 & 0.0827 & 0.9438 & 0.9419\\
NLM$^{16}_{0.35}$ & 27.3964 & 0.8273 & 0.9035 & 0.0827 & 0.9438 & 0.9419\\
NLM$^{16}_{0.5}$ & 27.3966 & 0.8273 & 0.9035 & 0.0827 & 0.9438 & 0.9419\\
NLM$^{16}_{0.65}$ & 27.4832 & 0.8311 & 0.9055 & 0.0817 & \bf{0.9441} & \bf{0.9422}\\
NLM$^{16}_{0.8}$ & 28.1533 & 0.8543 & 0.9175 & \bf{0.0793} & 0.9439 & \bf{0.9422}\\
NLM$^{16}_{0.9}$ & 28.6944 & \bf{0.8665} & \bf{0.9233} & 0.0850 & 0.9382 & 0.9368\\
NLM$^{16}_{1.0}$ & 28.9065 & 0.8640 & 0.9201 & 0.0988 & 0.9247 & 0.9235\\
\hline
\end{tabular}
\normalsize
\caption{Average image quality index for Gaussian noise, $\sigma=30$.}
\label{table:NLM_sigma30}
\end{center}
\end{table}


==> Tables/NLM_sigma40.tex <==
\begin{table}
\begin{center}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 & PSNR & SSIM & MSSSIM & GMSD & FSIM & FSIM$_C$ \\
\hline
noisy & 16.0903 & 0.4280 & 0.6414 & 0.2501 & 0.8157 & 0.7937\\
\hline
NLM$^{900}_{0.0}$ & \bf{27.7143} & 0.8184 & 0.8893 & 0.1303 & 0.8856 & 0.8844\\
NLM$^{16}_{0.0}$ & 25.3768 & 0.7522 & 0.8591 & 0.1061 & 0.9237 & 0.9206\\
\hline
NLM$^{16}_{0.1}$ & 25.3768 & 0.7522 & 0.8591 & 0.1061 & 0.9237 & 0.9206\\
NLM$^{16}_{0.2}$ & 25.3768 & 0.7522 & 0.8591 & 0.1061 & 0.9237 & 0.9206\\
NLM$^{16}_{0.35}$ & 25.3768 & 0.7522 & 0.8591 & 0.1061 & 0.9237 & 0.9206\\
NLM$^{16}_{0.5}$ & 25.3770 & 0.7522 & 0.8591 & 0.1061 & 0.9237 & 0.9206\\
NLM$^{16}_{0.65}$ & 25.4948 & 0.7580 & 0.8624 & 0.1043 & 0.9243 & 0.9213\\
NLM$^{16}_{0.8}$ & 26.3839 & 0.7942 & 0.8813 & \bf{0.0977} & \bf{0.9248} & \bf{0.9223}\\
NLM$^{16}_{0.9}$ & 27.1124 & \bf{0.8153} & \bf{0.8910} & 0.1037 & 0.9168 & 0.9148\\
NLM$^{16}_{1.0}$ & 27.4218 & 0.8147 & 0.8870 & 0.1214 & 0.8971 & 0.8954\\
\hline
\end{tabular}
\normalsize
\caption{Average image quality index for Gaussian noise, $\sigma=40$.}
\label{table:NLM_sigma40}
\end{center}
\end{table}

